Model Reduction of Shallow CNN Model for Reliable Deployment of Information Extraction from Medical Reports

Shallow Convolution Neural Network (CNN) is a time-tested tool for the information extraction from cancer pathology reports. Shallow CNN performs competitively on this task to other deep learning models including BERT, which holds the state-of-the-art for many NLP tasks. The main insight behind this eccentric phenomenon is that the information extraction from cancer pathology reports require only a small number of domain-specific text segments to perform the task, thus making the most of the texts and contexts excessive for the task. Shallow CNN model is well-suited to identify these key short text segments from the labeled training set; however, the identified text segments remain obscure to humans. In this study, we fill this gap by developing a model reduction tool to make a reliable connection between CNN filters and relevant text segments by discarding the spurious connections. We reduce the complexity of shallow CNN representation by approximating it with a linear transformation of n-gram presence representation with a non-negativity and sparsity prior on the transformation weights to obtain an interpretable model. Our approach bridge the gap between the conventionally perceived trade-off boundary between accuracy on the one side and explainability on the other by model reduction.

==> Makefile <==
##################################################
### COMMANDS

LATEX  = pdflatex --synctex=1
BIBTEX = bibtex

PERL   = perl

RM     = rm -rf
CD     = cd
MAKE   = make
MKDIR  = mkdir -p
MV     = mv
CP     = cp -r
ECHO   = @echo

SHELL = bash


##################################################
### DOCUMENT & OPTIONS

# document
DOC = main

# LaTeX compilation qualifiers
PLAIN     = \def\plain{true}
REVIEW    = \def\review{true}

##################################################
### CLEAN-UP EXTENSIONS

EXT_CLEAN = .tex~ .out .dvi .pdf .aux .toc .lof .lot .log .bbl .blg	\
	    .brf  .nav .snm .spl .glg .glo .gls .ist .idx .dep .ilg	\
	    .synctex.gz .run.xml -blx.bib Notes.bib

##################################################
### COMPILATION

# PHONY targets are always compiled
.PHONY: pdf update


# default "make" target
MAKEDEFAULT = draft
all: $(MAKEDEFAULT)

# ~~~~~~~~~~~~~~~~~~~~ GENERIC COMPILATION CORE

pdf: 
	$(LATEX) "$(OPTS)\input{$(DOC)}"
	$(BIBTEX) $(DOC)
	$(LATEX) "$(OPTS)\input{$(DOC)}"
	$(LATEX) "$(OPTS)\input{$(DOC)}"


# ==================== MANUSCRIPT

# ---------- plain

plain: OPTS += $(PLAIN)		## Plain format
plain: pdf

draft: plainreview
plainreview: OPTS += $(PLAIN) $(REVIEW) ## Draft
plainreview: pdf


clean:				## LaTeX output clean-up
	$(RM) $(addprefix $(DOC),$(EXT_CLEAN))
	$(RM) $(DOC)_revdiff-wrt-*.pdf
	$(RM) texput.log


help:				## Echo Makefile documentation
	@echo ""
	@grep -E '(^[a-zA-Z_-]+:.*?##.*$$)|(^# ====================)' $(MAKEFILE_LIST) | awk 'BEGIN {FS = ":.*?## "}{printf "\033[32m %-35s\033[0m %s\n", $$1, $$2}' | sed -e 's/\[32m # ====================/[33m===============/'
	@echo ""
	@echo -e "\e[033m*** REVISION SYNTAX:\e[0m \e[032mmake revision-xxx [REV=<svn-revision-num>]\e[0m"
	@echo ""
	@echo -e "\e[033m*** DEFAULT RULE:   \e[0m \e[032m$(MAKEDEFAULT)\e[0m"
	@echo ""


==> tex/acknowledgement.tex <==
%
This work has been supported in part by the Joint Design of Advanced
Computing Solutions for Cancer (JDACS4C) program established
by the U.S. Department of Energy (DOE) and the National
Cancer Institute (NCI) of the National Institutes of Health. This
work was performed under the auspices of the U.S. Department
of Energy by Argonne National Laboratory under Contract DEAC02-
06-CH11357, Lawrence Livermore National Laboratory under
Contract DEAC52-07NA27344, Los Alamos National Laboratory
under Contract DE-AC5206NA25396, and Oak Ridge National Laboratory
under Contract DE-AC05-00OR22725.

%
The authors wish to thank Valentina Petkov of the Surveillance
Research Program from the National Cancer Institute and the SEER
registries for providing the de-identified pathology reports. 
%The
%authors wish to thank Hong-Jun Yoon, Folami T. Alamudun, Mohammed Alawad, 
%Georgia Tourassi and Shang Gao at ORNL for sharing their expertise in the field 
%of study.


==> tex/lrp.tex <==
\section{Feature selection using LRP}
We use the Layer-wise Relevance Propagation (LRP)~\cite{??} for all documents to
locate the the important contributors to the prediction.
% 
Layer-wise Relevance Propagation (LRP) technique progagates the prediction  $\mathbf{f}(\mathbf{x})$ 
backwards in the neural network by means of propagation rules to acheive this. 
%
This is done by redistributing the relevance score to the lower layer while preserving
the following relation between the relevance scores in $\forall i, j$ layers and the class-label 
prediction, $\sum_{i} R_i = \sum_{j} R_j = \mathbf{f}(\mathbf{x})$.
%
The LRP algorithms vary in the mechanisms how the redistributing occurs.


==> tex/sensitivity.tex <==
%
\subsection{Sensitivity analysis}
\label{subsec:sensitivity-analysis}

In this section,...


==> tex/table-label-summary.tex <==
\begin{table}[tb]
  \centering
  \caption{Summary of label distribution in the de-identified pathology reports}
          {\normalsize
        %\small
        %\footnotesize
 \begin{tabular}{l p{125pt} c}
  \multicolumn{1}{c}{Label type} & (Labels, counts) & \#documents\\
  \hline
  Organ & (Lung, 504), (Breast, 521) & 1025\\
  ICD-O-3 code & (c34.0, 26), (c34.1, 139), (c34.2, 11), 
  (c34.3, 78), (c34.8, 6), (c34.9, 191), (c50.0, 1), 
  (c50.1, 13), (c50.2, 36), (c50.3, 10), (c50.4, 63), 
  (c50.5, 21), (c50.6, 2), (c50.9, 292) & 951\\
  Laterality & (bilateral, 6), (left, 400), (right, 415) & 821\\
  Behavior & (metastatic, 9), (in-situ, 101), (malignant, 910), (boderline, 1), (benign, 22) & 1043\\
  Grade & (grade 1, 124),  (grade 2, 233),  (grade 3, 271),  (grade 4, 17),  (grade 9, 1) & 646\\
\end{tabular}
 }
  \label{table:label-summary}
\end{table}


==> tex/workingnote.tex <==
%workingnote.tex

Date 01/02/2020: 

